Sensitivity Analysis of Individual Treatment Effects: A Robust Conformal Inference Approach

We propose a model-free framework for sensitivity analysis of individual treatment effects (ITEs), building upon ideas from conformal inference. For any unit, our procedure reports the $\Gamma$-value, a number which quantifies the minimum strength of confounding needed to explain away the evidence for ITE. Our approach rests on the reliable predictive inference of counterfactuals and ITEs in situations where the training data is confounded. Under the marginal sensitivity model of Tan (2006), we characterize the shift between the distribution of the observations and that of the counterfactuals. We first develop a general method for predictive inference of test samples from a shifted distribution; we then leverage this to construct covariate-dependent prediction sets for counterfactuals. No matter the value of the shift, these prediction sets (resp. approximately) achieve marginal coverage if the propensity score is known exactly (resp. estimated). We describe a distinct procedure also attaining coverage, however, conditional on the training data. In the latter case, we prove a sharpness result showing that for certain classes of prediction problems, the prediction intervals cannot possibly be tightened. We verify the validity and performance of the new methods via simulation studies and apply them to analyze real datasets.

==> sec5.tex <==
% !TEX root = paper.tex


The performance of the proposed procedures is demonstrated on simulated data. 
In Section~\ref{subsec:simu_predict}, we focus on counterfactual 
prediction to 
verify the validity and sharpness 
of the predictive inference procedures.
In Section~\ref{subsec:simu_sens}, 
we carry out sensitivity analysis to 
illustrate how the robustness of causal
conclusions can be assessed 
and how it relates
to the effect size and the confounding level. 

\subsection{Counterfactual prediction} \label{subsec:simu_predict}

% In this part, we focus on counterfactual prediction with Algorithms~\ref{alg:mgn}
% and~\ref{alg:whp} given the true confounding level. 
% We work with $Y(1)$ 
% from the super-population, i.e., the ATE-type inference. 
% % \subsubsection{Simulation settings}
% % \label{sec:sim_setup}
% % In the experiments, we will fix a super-population to generate all random variables.
% % Then for various confounding levels $\Gamma \geq 1$, 
% % treatment assignments are generated 
% % from some mechanism satisfying~\eqref{eq:gamma_sel_mgn}, 
% % leading to different observed distributions of $(X,Y,T)$. 
% To demonstrate the validity, 
% we run the procedures with the same level $\Gamma$
% as the data generating process. 

%\paragraph{Data generating process}
We fix a super-population model similar to the 
setting in~\cite{yadlowsky2018bounds}. 
Given a sample size $n_\train = n_\calib \in \{500, 2000,5000\}$
and a covariate dimension $p\in\{4,20\}$, we generate the covariates 
and unobserved confounders with 
\$
X\sim \textrm{Unif}[0,1]^p,\quad U\given X \sim N\Big(0,1+\frac{1}{2} \cdot (2.5X_1)^2\Big).
\$
The counterfactual of interest is $Y(1)$ generated as 
\$
Y(1) = \beta^\top X + U,\quad \textrm{where}~~ \beta = (-0.531, 0.126, -0.312, 0.018,0,\dots,0)^\top \in \RR^p.
\$ 
In other words, the fluctuation of $Y(1)$ from 
its conditional mean is entirely driven by $U$. 
With i.i.d.~data $(X_i,Y_i,U_i)$ 
generated from the fixed super-population, 
treatment assignments $T_i$ are generated from 
treatment mechanisms satisfying~\eqref{eq:gamma_sel_mgn}
with different confounding levels $\Gamma\in\{1,1.5,2,2.5,3,5\}$. 
% Here $\Gamma=1$ corresponds to the strong ignorability condition 
% as in~\cite{lei2020conformal}. 
Specifically, we design the propensity scores as
\#\label{eq:simu_prop}
e(x) = \text{logit}(\beta^\top x),\quad e(x,u) = a(x) \ind\{|u|>t(x)\} + b(x) \ind\{|u|\leq t(x)\},
\#
for the same $\beta\in \RR^p$. Above,
\$
a(x) = \frac{e(x)}{e(x) + \Gamma(1-e(x))},\quad b(x) = \frac{e(x)}{e(x) +  (1-e(x))/\Gamma}
\$ 
are the lower and upper bounds on $e(x,u)$ under the marginal $\Gamma$-selection model. 
The threshold $t(x)$ is designed to ensure $\EE[e(X,U)\given X] = e(X)$. 
% We then generate $T_i \given X_i,U_i \sim \textrm{Bern}(e(X_i,U_i))$. 
The training data $\cD$ are $\{(X_i,Y_i(1)\}$ for those $T_i=1$.
% This setting shows how, for a fixed population, 
% the observations and predictions 
% would change with selection mechanisms 
% under different confounding levels. 
By~\eqref{eq:simu_prop}, the setting is designed to be adversarial 
so as to show the performance of our method in a nearly worst case. 

%\paragraph{Implementation details}
For each configuration of $(n_\calib,p,\Gamma,\alpha)$, 
we run Algorithm~\ref{alg:mgn} and~\ref{alg:whp} %$N=1000$ times,
both with ground truth $\ell(\cdot)$, $u(\cdot)$ 
and with estimated $\hat{\ell}(\cdot)$, $\hat{u}(\cdot)$. 
To obtain estimated bound functions, 
we fit the propensity score $\hat{e}(x)$ on $\cD_\train$ 
using regression forests from the \texttt{grf} R-package,
and set $\hat{\ell}(x) = \hat{p}_1 (1+ (1-\hat{e}(x))/(\Gamma\cdot \hat{e}(x)))$,
$\hat{u}(x) = \hat{p}_1 (1+\Gamma\cdot (1-\hat{e}(x))/\hat{e}(x))$
with $\hat{p}_1$ being the empirical proportion of $T_i=1$. 
For Algorithm~\ref{alg:mgn},
we compute the average coverage on one test sample 
over $N=1000$ independent runs.
For Algorithm~\ref{alg:whp},
we evaluate the empirical coverage on $10000$ test samples 
for all $N=1000$ independent runs. 



The proposed approaches work for any nonconformity score function
and any training method. 
In our experiments, we follow the  
Conformalized Quantile Regression algorithm (CQR)~\citep{romano2019conformalized}
to compute the nonconformity score: 
$\cD_\train$ is employed to train a 
conditional quantile function $\hat{q}(x,\beta)$
for $Y(1)$ conditional on $X$ 
by quantile random forests~\citep{meinshausen2006quantile}.
Then for \revise{a target level} $\alpha\in(0,1)$, the 
nonconformity score is defined as
\$
V(x,y) = \max \big\{ \hat{q}\,(x,\alpha/2) - y, ~y - \hat{q}\,(x,1-\alpha/2)\big\}.
\$
We run the procedures for a target $\alpha \in \{0.1,0.2,\dots,0.9\}$
with the corresponding nonconformity scores. 
For Algorithm~\ref{alg:whp}, we keep $\delta=0.05$
and  employ the W-S--R bound 
as in Proposition~\ref{prop:wsr_bound}. 

\subsubsection{Results of the marginally valid procedure}

% We present the performance of the predictive interval 
% provided by Algorithm~\ref{alg:mgn} over $N=1000$ replicates
% when $\hat \ell(\cdot)$ and $\hat u(\cdot)$
% are estimated. 
%For comparison, we 

%which is Algorithm~\ref{alg:mgn} with $\Gamma=1$ for all confounding levels.
The empirical coverage 
when $\hat \ell(\cdot)$ and $\hat u(\cdot)$ are estimated 
is summarized in Figure~\ref{fig:mgn_cov_est},
with its counterpart with ground truth in Figure~\ref{fig:mgn_cov_known}
in Appendix~\ref{app:simu_predict} showing quite similar performance.  
% In these simulations, we also implemented 
% the vanilla counterfactual inference procedure~\citep{lei2020conformal} 
% show the necessity of adjusting for confounders.


\begin{figure}[h]
\centering 
\includegraphics[width=5.5in]{figs/marginal_estimated_coverage.pdf}
\caption{Empirical coverage of Algorithm~\ref{alg:mgn} when $\hat \ell(\cdot)$
and $\hat u(\cdot)$ are estimated. Each column corresponds to a sample size $n = n_\calib$,
while each row corresponds to a dimension $p$. Within each subplot, 
each line corresponds to a confounding level $\Gamma$. 
The solid lines are for Algorithm~\ref{alg:mgn}.
\revise{The dashed lines assume no confounding 
and are shown for comparison.}
%in~\cite{lei2020conformal}. 
}
\label{fig:mgn_cov_est}
\end{figure}
    

\paragraph{Validity} 
In Figure~\ref{fig:mgn_cov_est}, 
the solid lines are all above the $45^\circ$-line, 
showing the validity of the proposed procedure 
over the whole spectrum of sample sizes. We also see that confounding
must be taken into consideration to reach valid counterfactual
conclusions.  
% On the contrary, the vanilla procedure, represented by 
% the dashed lines, fail to cover the counterfactual
% since it does not account for confounding. 


\paragraph{Sharpness}
In all the configurations, especially 
when the target coverage is close to $0.5$, 
the actual coverage is quite close to the target, 
which shows the sharpness of the prediction interval 
in this setting.  


\paragraph{Robustness to estimation error} 
The valid coverage also shows robustness to the estimation error. 
As illustrated in the decomposition~\eqref{eq:mgn_gap_decomp},
the gap between $\ell(x)$ and $w(x,y)$ (as well as  
that between $w(x,y)$ and $u(x)$) 
provides some buffer for the estimation error
in $\hat{\ell}(\cdot)$ and $\hat{u}(\cdot)$. 
To be concrete, we numerically evaluate 
the gap $\hat\Delta$
with $(q,p) = (\infty,1)$ 
as well as the estimation error
$\|\hat{\ell}(X)-\ell(X)\|_1$ and $\|\hat{u}(X)-u(X)\|_1$. 
The results are summarized in Figure~\ref{fig:mgn_gap}. 
We see that although the estimation error of the 
lower and upper bounds can sometimes be large, 
\revise{the realized gap $\hat\Delta$} is often very close to zero.

\begin{figure}[H]
\centering 
\includegraphics[width=1\linewidth]{figs/mgn_gap_add.pdf}
\caption{Empirical gap and estimation errors. The plots in 
the second row zoom in on the gaps. 
Each plot corresponds to a sample size $n = n_\calib$ and a dimension $p$. 
The long-dashed lines are $\|\hat{u}(X)-u(X)\|_1$,
the short-dashed lines are $\|\hat{\ell}(X)-\ell(X)\|_1$, and
the solid lines are 
$\hat\Delta$ defined in Theorem~\ref{thm:mgn}.}
\label{fig:mgn_gap}
\end{figure}


\subsubsection{Results of the PAC-type procedure}
To verify the PAC-type guarantee %~\eqref{eq:pac_target} 
of Algorithm~\ref{alg:whp},
we compute the $0.05$-th quantile of realized empirical coverage 
of the $N=1000$ replicates and compare it to the target level $1-\alpha$. 
% We do not compare with the procedure in \cite{lei2020conformal} since
% there is no counterparts with this type of guarantee. 
The results with estimated $\hat{\ell}(\cdot)$ and $\hat{u}(\cdot)$ are 
summarized in Figure~\ref{fig:whp_qt_est}, and those  
with ground truth of $\ell(\cdot)$ and $u(\cdot)$ 
%deferred to 
in Figure~\ref{fig:whp_qt_known} in Appendix~\ref{app:simu}. 
The marginal coverage 
is presented in Figures~\ref{fig:whp_cov_known} and~\ref{fig:whp_cov_est}
in Appendix~\ref{app:simu_predict}.  

\begin{figure}[htbp]
\centering 
\includegraphics[width=5in]{figs/whp_est_cov_quantile.pdf}
\caption{$0.05$-th quantile of empirical coverage 
in Algorithm~\ref{alg:whp} when $\hat \ell(\cdot)$
and $\hat u(\cdot)$ are estimated. 
Each figure corresponds to a configuration of 
sample size $n = n_\calib$
and dimension $p$. Within each subplot, 
each line corresponds to a confounding level $\Gamma$. }
\label{fig:whp_qt_est}
\end{figure}

% \noindent \textbf{Validity}
\paragraph{Validity}
In Figure~\ref{fig:whp_qt_est}, 
the $0.05$-th quantiles of empirical coverage   
all lie above the $45^\circ$-line,
% of target levels, 
which confirms 
the validity of the proposed procedure.  
% In Figure~\ref{fig:whp_qt_known}
% where $\hat\ell(\cdot)$ and $\hat{u}(\cdot)$ are known, 
% the quantiles are always larger
% than the target as well. \\

% \noindent \textbf{Sharpness}
\paragraph{Sharpness}
The quantile-versus-target lines in Figure~\ref{fig:whp_qt_est}
almost overlap with the $45^\circ$-line, since by design
the data generating distribution is a near-worst case.
%show the sharpness of the procedure 
%with the near-worst case by design. 
This shows the sharpness of our method and
is in accordance with the theoretical justification 
in Section~\ref{subsec:sharp}. 
%The regions where the target coverage is close to $0.5$ 
%is a little bit loose with $n=500$, 
%which is due to the nature of the Waudby-Smith--Ramdas bound. 

% \noindent \textbf{Robustness to estimation error}
\paragraph{Robustness to estimation error}
Similar to Algorithm~\ref{alg:mgn},
the PAC-type algorithm shows robustness to the 
estimation error. 
In Figure~\ref{fig:whp_gap},
we numerically evaluate  the 
gap $\hat\Delta$ in~\eqref{eq:whp_gap} as well as 
the estimation errors 
$\|\hat{\ell}(X)-\ell(X)\|_1$ and $\|\hat{u}(X)-u(X)\|_1$. 
Even though the estimations error (dashed lines)
can be nonnegligibly off, 
the actual gap $\hat\Delta$  defined in Theorem~\ref{thm:whp}
is small. 




\begin{figure}[h]
\centering 
\includegraphics[width=1\linewidth]{figs/whp_gap.pdf}
\caption{Empirical gap and estimation errors. The plots in the 
second row zoom in on the gaps. 
Each plot corresponds to a sample size $n = n_\calib$ and a dimension $p$. 
The long-dashed lines are $\|\hat{u}(X)-u(X)\|_1$,
the short-dashed lines are $\|\hat{\ell}(X)-\ell(X)\|_1$, and
the solid lines are $\hat\Delta$ defined in Theorem~\ref{thm:whp}.}
\label{fig:whp_gap}
\end{figure}

 


\subsection{Sensitivity analysis} \label{subsec:simu_sens}
%The simulations on sensitivity analysis 
We focus on the ATT-type inference for the directional null 
\$
H_0(\Gamma)\colon Y(1)-Y(0)\leq 0~~\text{and}~~ \PP^\super\in \cP(\Gamma).
\$
The test sample is from $\PP_{X,Y(0),Y(1)\given T=1}$,
\revise{for which we observe $(X_{n+1},Y_{n+1}(1))$ 
and would like to predict $Y_{n+1}(0)$.} 

We fix $n_\train = n_\calib = 2000$ and $p=4$. 
The covariates $X$, unobserved confounders $U$
and counterfactual $Y(0)$ (instead of $Y(1)$) are generated 
in
the same way as in Section~\ref{subsec:simu_predict}. 
The treatment mechanism $e(x,u)$ is also the same as in~\eqref{eq:simu_prop}
with confounding level $\Gamma \in \{1.2, 1.4, \dots, 2\}$. 
The training data are $(X_i,Y_i(0))$ for those $T_i=0$. 
We generate $Y(1)$ in two ways: 1) $Y (1)-Y (0)\equiv a$ (fixed ITE) and 
2) $Y(1) - Y(0) = a\cdot U$ (random ITE). Here  $a$ ranges in  
$\{-1,-0.5, 0, 0.5, 1\}$. 

Fixing level $\alpha = 0.1$ and $\delta=0.05$ (for Algorithm~\ref{alg:whp}), 
for each fixed  $\Gamma\geq 1$, we construct a
one-sided ATT-type prediction interval for $Y(0)$, 
which takes the form $\hat{C}(X_{n+1},\Gamma) = (-\infty, \hat{Y}(X_{n+1},\Gamma)]$.
%for $Y(0)$  
%is constructed 
%utilizing 
The prediction interval is obtained 
via the non-conformity score 
\#\label{eq:score_oneside_cqr}
V(x,y) = y - \hat{q} (x,1-\alpha).
\# 
%The conditional quantile function $\hat{q}(\cdot,\cdot)$ is
%estimated in the same way 
%obtained 
%in the same way as Section~\ref{subsec:simu_predict}. 
We reject no hypotheses if $Y_{n+1}(1) \leq \hat{Y}(X_{n+1},1)$;
otherwise, we
reject all $H_0(\Gamma)$ such that $Y_{n+1}(1) > \hat{Y}(X_{n+1},\Gamma)$,  
hence the rejection set is $\cR = [1, \hat\Gamma)$ for some $\hat\Gamma>1$, 
which we define as the $\Gamma$-value. 
% When we make no rejection, we designate the $\Gamma$-value to be zero 
% in the plots. 


% \subsubsection{Discovery: the impact of true effect and confounding}
% We first take a moment to illustrate the impact of 
% true effect size and confounding level on 
% the inference of ITE 
% when we fail to account for confounding. 
% To be specific, 
% we keep track of \emph{true discovery}\footnote{If the ITE is fixed at $a \leq 0$, the hypotheses $H_0(\Gamma)$ are always true, 
% so we do not track it. }, 
% defined as the frequency of 
% making any rejection and $Y(1)-Y(0)>0$. 
% The results are summarized in Figure~\ref{fig:simu_ss_disc},
% where  
% larger true effects 
% and higher confounding level make  it easier to 
% make any true rejection on negative ITE. 

% \begin{figure}[H]
% \centering
% \begin{subfigure}[t]{0.24\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figs/mest_fixed_disc_mean.pdf}
%     \caption{ Alg.\ref{alg:mgn}, fixed ITE  } 
% \end{subfigure}
% \begin{subfigure}[t]{0.24\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figs/mest_random_disc_mean.pdf}
%     \caption{ Alg.\ref{alg:mgn}, random ITE }  
% \end{subfigure}
% \begin{subfigure}[t]{0.24\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figs/west_fixed_disc_mean.pdf}
%     \caption{ Alg.\ref{alg:whp}, fixed ITE  } 
% \end{subfigure}
% \begin{subfigure}[t]{0.24\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figs/west_random_disc_mean.pdf}
%     \caption{ Alg.\ref{alg:whp}, random ITE }  
% \end{subfigure}
% \caption{Discovery at any confounding level  for fixed  random ITE using procedures with estimated $\hat\ell(\cdot)$ and $\hat{u}(\cdot)$. 
% The solid lines are empirical averages. The shaded areas are the 
% $0.25$ and $0.75$ quantiles. }\label{fig:simu_ss_disc}
% \end{figure}


% However, 
% the `fake' effects 
% driven by confounding 
% often comes with increased \emph{false discovery} as well---
% we also evaluate the frequency of 
% rejecting any $H_0(\Gamma)$ (i.e., rejecting $H_0(1)$) and $Y(1)-Y(0)\leq 0$ 
% in Figure~\ref{fig:simu_ss_disct}.

% \begin{figure}[H]
% \centering
% \begin{subfigure}[t]{0.24\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figs/mest_fixed_tdisc_mean.pdf}
%     \caption{ Alg.\ref{alg:mgn}, fixed ITE  } 
% \end{subfigure}
% \begin{subfigure}[t]{0.24\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figs/mest_random_tdisc_mean.pdf}
%     \caption{ Alg.\ref{alg:mgn}, random ITE }  
% \end{subfigure}
% \begin{subfigure}[t]{0.24\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figs/west_fixed_tdisc_mean.pdf}
%     \caption{ Alg.\ref{alg:whp}, fixed ITE  } 
% \end{subfigure}
% \begin{subfigure}[t]{0.24\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figs/west_random_tdisc_mean.pdf}
%     \caption{ Alg.\ref{alg:whp}, random ITE }  
% \end{subfigure}
% \caption{False discovery at any confounding level for fixed  and random ITE using procedures with estimated $\hat\ell(\cdot)$ and $\hat{u}(\cdot)$. 
% The solid lines are empirical averages. The shaded areas are the 
% $0.25$ and $0.75$ quantiles.}\label{fig:simu_ss_disct}
% \end{figure}

% In words, Figures~\ref{fig:simu_ss_disc} and~\ref{fig:simu_ss_disct} 
% show how higher confounding level leads to more discoveries, 
% both true and false, if we do not account for possible confounding. 
% Such risk could be overcomed by our sensitivity analysis framework, 
% where  rigorous assessment of 
% the robustness of inference on ITE is available. 

\subsubsection{FWER control} 

We evaluate the empirical FWER, which is the proportion of making a false rejection
among $\{H_0(\Gamma)\}_{\Gamma\geq 1}$, 
averaged over all test samples in all $N=1000$ independent runs.  
The results with estimated $\hat{\ell}(\cdot)$ and $\hat{u}(\cdot)$ are presented
in Figure~\ref{fig:simu_ss_fwer}, where
we omit the case of fixed ITE 
at $a > 0$ since the hypotheses $H_0(\Gamma)$ are always false.
Figure~\ref{fig:simu_ss_fwer} shows control of 
the FWER even when the 
likelihood ratio bounds are estimated. 
The results with the ground truth $\ell(\cdot)$ and $u(\cdot)$ 
are in Appendix~\ref{app:simu_sens}.


\begin{figure}[H]
\centering
\begin{subfigure}[t]{0.24\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/mest_fixed_fwer_mean.pdf}
    \caption{ Alg.\ref{alg:mgn}, fixed ITE  } 
\end{subfigure}
\begin{subfigure}[t]{0.24\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/mest_random_fwer_mean.pdf}
    \caption{ Alg.\ref{alg:mgn}, random ITE }  
\end{subfigure}
\begin{subfigure}[t]{0.24\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/west_fixed_fwer_qt.pdf}
    \caption{ Alg.\ref{alg:whp}, fixed ITE  } 
\end{subfigure}
\begin{subfigure}[t]{0.24\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/west_random_fwer_qt.pdf}
    \caption{ Alg.\ref{alg:whp}, random ITE }  
\end{subfigure}
\caption{Empirical FWER with estimated $\hat\ell(\cdot)$ and $\hat{u}(\cdot)$
with the effect size $a$ ranging in $\{-1,-0.5,0,0.5,1\}$. 
In (a,b), the solid lines are averaged over $N=1000$ runs, while the $0.25$-th 
and $0.75$-th quantiles form
the shaded area. 
In (c,d), the solid lines are the $0.05$-th quantile of $N=1000$ runs.}\label{fig:simu_ss_fwer}
\end{figure}


\subsubsection{\revise{$\Gamma$-values} }
% To visualize the results, w
We plot the 
estimated survival function $\hat \Gamma$
defined as $S(\Gamma) =  \PP(\hat{\Gamma} > \Gamma)$, 
which  
characterizes the proportion of test units 
that are identified as positive ITE 
with each confounding level $\Gamma$.
Figure~\ref{fig:simu_gval_mgn} presents
the results from  one run of the procedure
with Algorithm~\ref{alg:mgn},
where we focus on the random ITE: $Y(1)-Y(0)=a\cdot U$.
%Equivalently, 
%it is the proportion of units 
%whose $\Gamma$-values are above each 
%confounding level $\Gamma$. 


%The empirical c.d.f.~is a description of 
%the distribution of $\Gamma$-values and



\begin{figure}[H]
\includegraphics[width=\linewidth]{figs/mgn_gvalue.pdf}
\caption{
%Proportion of the test units identified as positive ITEs 
%with confidence level $1-\alpha=0.9$
%at various confounding levels, 
Empirical evaluation of $S(\Gamma)$
reported by (one run of) the sensitivity analysis procedure with Algorithm~\ref{alg:mgn}. The red dashed vertical lines are the true confounding levels.}
\label{fig:simu_gval_mgn}
\end{figure}

% Take the case of true confounding level $\Gamma = 1.6$ and $a = 1$ for example
% (the brown curve in the fourth plot).
% There are approximately $15\%$ of the samples
% whose $\Gamma$-values are above
% $2.5$---this means for each of these samples, 
% we have $90\%$ confidence that 
% there is a positive ITE
% unless the confounding level is more than $2.5$. 


% The empirical c.d.f.~provides an 
% approximation to the distribution 
% of the invididual $\Gamma$-value. 
To see how to interpret these plots,
let us consider the example where
$a = 1$ and the true confounding level
is $1.6$. We can see that around $10\%$ of the 
samples have a $\Gamma$-value greater
than $2.5$, and $5\%$ have a $\Gamma$-value
greater than $5$, showing strong evidence
for positive ITEs.
Note also that the ITE is always zero when $a=0$, 
and the $\Gamma$-value should be a $90\%$ lower confidence 
bound for the true confounding level. In Figure~\ref{fig:simu_gval_mgn},
we indeed observe that for around $90\%$ of the samples,
the $\Gamma$-value is below the true confounding level (see the
green curves).




With random ITEs, 
both 
the magnitude of actual ITE  
and % increases with the effect size $a$, 
the gap between observed outcomes in treated and control groups
increase  with the effects size $a$.
%leading to complicated influence of confounding 
%on the inference. 
Within each subplot, 
the reported  $\Gamma$-values become larger
as the effect size increases.  
Thresholding at the true confounding level $\Gamma$, we see that 
larger magnitude of true effects also makes it easier to detect 
positive ITEs at the correct confounding level $\Gamma$. 
%On the other hand, for each fixed effect size, 
%the reported $\Gamma$-values become larger 
%as the increased confounding level 
%shifts the predictive intervals left. 
%However, %if we threshold each subplot at the true confounding level $\Gamma$, 
%the proportion of rejection at the true confounding level 
%does not necessarily increase with the confounding level. 


%When we compare the results across settings,
%%we see for a fixed effect size, the
%$\Gamma$-values become larger 
%as the confounding level increases.
%This is because in our adversarial design, 
%unmeasured confounding shifts the observed distribution, 
%hence the predictive interval for $Y(0)$, to be smaller.  
%Consequently, there is a larger gap 
%between the treated and control outcomes---that is, 
%the unmeasured confounding creates `fake' effects. 
%On the other hand, since $Y(1)-Y(0)=a\cdot U$, 
%larger effect size $a$ increases  
%the magnitude of the ITE and creates true effects. 
%The unmeasured confounder $U$ influences 
%the output of the sensitivity procedure 
%in two mixed ways. 


The results
from one run of Algorithm~\ref{alg:whp} \revise{are} 
in Figure~\ref{fig:simu_gval_whp}. 
The patterns are 
similar to \revise{Figure~\ref{fig:simu_gval_mgn}}
in general, 
except that it is sometimes sharper than Algorithm~\ref{alg:mgn} 
and provides slightly stronger evidence 
against unmeasured confounding. 


\begin{figure}[H]
\includegraphics[width=\linewidth]{figs/whp_gvalue.pdf}
\caption{
%Proportion of the test units identified as positive ITEs 
%with confidence level $1-\alpha=0.9$
%at various confounding levels,  
Empirical evaluation of $S(\Gamma)$ reported by 
(one run of) the sensitivity analysis procedure with Algorithm~\ref{alg:whp}. The red dashed vertical lines are the true confounding levels.}
\label{fig:simu_gval_whp}
\end{figure}


In Figure~\ref{fig:simu_gval_whp}, 
some test units have large $\Gamma$-values 
especially when the effect size is positive. 
Such strong evidence would happen if 
there is a \revise{large} gap between the observed $Y(1)$
and the typical behavior of $Y(0)$
\revise{predicted with} the training data---thus, 
the only way our procedures can 
output a prediction interval that overlaps with $Y(1)$
is  $\hat{C}(X,\Gamma) = \{V(X,y)\leq \hat{v}\} =\RR$, 
where $\hat{v}=\infty$. 
In that case, 
there is a certain value $\Gamma_\infty(X)$ 
such that $\hat{v}=\infty$ once $\Gamma \geq \Gamma_\infty(X)$. 
Since 
Algorithm~\ref{alg:whp} outputs a same $\hat{v}$ for 
all test samples, 
the value $\Gamma_\infty$ is the same 
for all such extreme individuals,
leading to steep tails 
in Figure~\ref{fig:simu_gval_whp}. 
In contrast, 
Algorithm~\ref{alg:mgn} returns 
different $\Gamma_\infty(X)$ 
for different individuals, 
\revise{and produces a smoother
curve (Figure~\ref{fig:simu_gval_mgn}).}

\subsubsection{False discovery proportions}

\revise{We also track the empirical false discovery proportion 
% among test units that survive a certain confounding level, i.e., 
\$
\text{FDP}(\Gamma) = \frac{ \big|\{j\in \cD_{\test} \colon \hat\Gamma > \Gamma, ~
Y_j(1)\leq Y_j(0)\} \big| }{  \big|\{j\in \cD_{\test} \colon \hat\Gamma > \Gamma\} \big| },
\quad \Gamma\geq 1
\$
for random ITE with $a\neq 0$, 
which is the proportion of false rejections 
among test units that are rejected at confounding level $\Gamma$. 
With both the two procedures, 
we find that $\text{FDP}(\Gamma)$ is always zero---the
units that survive certain levels of adjustment for confounding 
all have positive ITE. 
It could be explained by the conservativeness of the procedure: 
to survive the adjustment, 
the observed $Y(1)$ needs to be
larger than the whole $1-\alpha$ prediction interval 
for $Y(0)$.
Therefore, a unit that survives the adjustment 
is much more likely 
to have a positive ITE, leading to vanishing FDPs.

% The behavior of FDP relies on the 
% dependence between predictive intervals for $Y(0)$ 
% and the unidentifiable ITE. 
}

% In words, for some individuals, there is an extremely large 
% difference between the observed $Y(1)$ 
% and the typical behavior of $Y(0)$ as suggested by the predictive interval, 
% showing a strong evidence of positive ITEs. 


% \subsubsection{Power illustration}
% Finally, we evaluate the \emph{power}, defined 
% as the frequency of rejecting $Y(1)-Y(0)\leq 0$ at the correct confounding level, 
% i.e., rejecting $H_0(\Gamma^*)$ and $Y(1)-Y(0)>0$. 
% The results are summarized in Figure~\ref{fig:simu_ss_power}. 


% \begin{figure}[H]
% \centering
% \begin{subfigure}[t]{0.24\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figs/mest_fixed_power_mean.pdf}
%     \caption{ Alg.\ref{alg:mgn}, fixed ITE  } 
% \end{subfigure}
% \begin{subfigure}[t]{0.24\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figs/mest_random_power_mean.pdf}
%     \caption{ Alg.\ref{alg:mgn}, random ITE  } 
% \end{subfigure}
% \begin{subfigure}[t]{0.24\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figs/west_fixed_power_mean.pdf}
%     \caption{ Alg.\ref{alg:whp}, fixed ITE  } 
% \end{subfigure}
% \begin{subfigure}[t]{0.24\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figs/west_random_power_mean.pdf}
%     \caption{ Alg.\ref{alg:whp}, random ITE  } 
% \end{subfigure}
% \caption{Power for fixed and random ITE with using procedures with estimated $\hat\ell(\cdot)$ and $\hat{u}(\cdot)$. 
% The solid curves are averaged values for various effect sizes $a$. 
% The 0.25 and 0.75 quantiles form the shaded area.  }\label{fig:simu_ss_power}
% \end{figure}

% As illustrated in Figure~\ref{fig:simu_ss_power},
% in our setting, 
% confounding actually makes it harder to 
% identify positive ITEs at the correct robustness level. 
% However, 
% with our sensitivity analysis procedure, 
% we still have 
% reliable quantification of robustness
% as illustrated 
% by the FWER control. 



% \subsubsection{Sensitivity analysis with marginally valid procedure}
% \label{subsubsec:simu_sens_mgn}

% Fixing the coverage target at $1-\alpha=0.9$, 
% % for each configuration of fixed effect $a$ and confounding level $\Gamma$, 
% % Algorithm~\ref{alg:mgn} is used to provide marginally valid 
% % ATT-type predictive intervals of the form  
% % $\hat{C}(X_{n+1},\Gamma) = (-\infty, \hat{Y}(X_{n+1},\Gamma)]$ 
% % for $Y_{n+1}(0)$ given $T_{n+1}=1$. 
% we repeat the procedure $N=1000$ times for 
% each fixed effect $a$ and confounding level $\Gamma$, 
% each with $n_\test=500$
% test samples. 

% We evaluate the empirical FWER as the proportion of making a false rejection, 
% averaged over all test samples in all replicates.  
% If the ITE is fixed at $a > 0$, the hypotheses $H_0(\gamma)$ are always false, 
% hence we do not track the FWER. 
% The results with estimated $\hat{\ell}(\cdot)$ and $\hat{u}(\cdot)$ are presented
% in Figure~\ref{fig:simu_ss_mest}.


% \begin{figure}[htbp]
% \centering
% \begin{subfigure}[t]{0.43\linewidth}
%     \centering
%     \includegraphics[height=2in]{figs/mest_fixed_fwer_mean.pdf}
% \end{subfigure}
% \begin{subfigure}[t]{0.43\linewidth}
%     \centering
%     \includegraphics[height=2in]{figs/mest_random_fwer_mean.pdf}
% \end{subfigure}
% \caption{Empirical FWER for fixed ITE (left) and random ITE (right) with marginally-valid procedure.
% The averaged values are 
% the solid curves in the plots corresponding to various effect sizes $a$. 
% We also take the 0.25 and 0.75 quantiles of $N=1000$ runs of FWER, %power and discovery on test samples, 
% which is 
% the shaded area. }\label{fig:simu_ss_mest}
% \end{figure}

% Figure~\ref{fig:simu_ss_mest} shows the valid control of FWER even when the 
% likelihood ratio bounds are estimated. 
% For smaller value of effect size, 
% it is harder for the procedure to make false rejections 
% since the observed $Y(1)$ gets closer to the predictive interval of $Y(0)$. 






% \begin{figure}[htbp]
% \centering
% \begin{subfigure}[t]{0.24\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figs/mest_fixed_power_mean.pdf}
%     \caption{ Power (fixed ITE) } 	 
% \end{subfigure}
% \begin{subfigure}[t]{0.24\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figs/mest_random_power_mean.pdf}
%     \caption{ Power (random ITE) }  
% \end{subfigure}
% \begin{subfigure}[t]{0.24\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figs/mest_fixed_disc_mean.pdf}
%     \caption{ Discovery (fixed ITE) } 
% \end{subfigure}
% \begin{subfigure}[t]{0.24\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figs/mest_random_disc_mean.pdf}
%     \caption{ Discovery (random ITE) }  
% \end{subfigure}
% \caption{Power (a-b) and discovery (c-d) for fixed ITE and random ITE with marginally-valid procedure.}\label{fig:simu_ss_mest_power}
% \end{figure}


% The discovery curves of (c-d) in Figure~\ref{fig:simu_ss_mest_power}
% show that larger confounding and larger effect size 
% drives larger witnessed discrepancy between the two outcomes, 
% leading to more discoveries of positive ITEs. 
% However, 
% confounding still makes it harder
% ---
% for the random ITE case where the ITE is also confounded, 
% under the difficult setting of $a<0$, 
% even though the ITE can be 
% positive with probability $0.5$, 
% we still make no discovery
% at the $0.9$ confidence level.  

% On the other hand, 
% as seen in (a-b),
% % the ability to identify positive ITEs at the correct 
% % confounding level (power) does not necessarily follow this pattern. 
% in our setting, 
% confounding actually makes it harder to 
% identify positive ITEs at the correct robustness level. 
% However, 
% with our sensitivity analysis procedure, 
% we still have 
% reliable quantification of robustness
% as illustrated 
% by the FWER control. 





% \subsubsection{Sensitivity analysis with PAC-type procedure}

% We fix the coverage target at $1-\alpha=0.9$
% and confidence level at $\delta = 0.05$. 
% For any configuration of $(a,\Gamma)$, 
% we employ Algorithm~\ref{alg:whp} to obtain PAC-type one-sided 
% predictive intervals $\hat{C}(X_{n+1},\Gamma) = (-\infty, \hat{Y}(X_{n+1},\Gamma)]$ 
% for $Y_{n+1}(0)$ given $T_{n+1}=1$. 
% For each of $n_\test = 10000$ test samples, we invert the predictive intervals to 
% obtain $\hat\Gamma$ as the smallest $\gamma$ such that 
% the observed $Y_{n+1}(1)<\hat{Y}(X_{n+1},\gamma)$. 

% In each replicate,
% we evaluate the empirical FWER as the proportion of making a false rejection.
% % The theoretical results in Section~\ref{sec:sens_analysis} 
% % guarantee that the $0.95$ quantile of all $N=1000$ FWERs is below $\alpha=0.1$. 
% We report the empirical $0.95$ quantiles in Figure~\ref{fig:simu_ss_west}
% for different configurations of effect and confounding level
% where the bound functions are estimated.
% The valid control of FWER in Figure~\ref{fig:simu_ss_west} 
% verifies the theoretical results in Section~\ref{sec:sens_analysis}
% up to estimation errors in the bound functions. 

% \begin{figure}[htbp]
%     \centering
%     \begin{subfigure}[t]{0.43\linewidth}
%         \centering
%         \includegraphics[height=2in]{figs/west_fixed_fwer_qt.pdf}
%         % \caption{ FWER (fixed ITE) } 	 
%     \end{subfigure}
%     \begin{subfigure}[t]{0.43\linewidth}
%         \centering
%         \includegraphics[height=2in]{figs/west_random_fwer_qt.pdf}
%         % \caption{ FWER (random ITE) } 
%     \end{subfigure}
%     \caption{Empirical FWER for fixed ITE (left) and random ITE (right) with PAC-type procedure.}\label{fig:simu_ss_west}
%     \end{figure}




% In all cases, we also evaluate the mean power and discovery
% averaged over all test samples of all replicates 
% to illustrate the relation to confounding levels and effect sizes. 
% The results are summarized in Figure~\ref{fig:simu_ss_west_power}.
% % The results with estimated $\hat{\ell}(\cdot)$ and $\hat{u}(\cdot)$ 
% % are summarized in Figure~\ref{fig:simu_ss_west_power}.


% \begin{figure}[htbp]
% \centering
% \begin{subfigure}[t]{0.24\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figs/west_fixed_power_mean.pdf}
%     \caption{ Power (fixed ITE) } 	 
% \end{subfigure}
% \begin{subfigure}[t]{0.24\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figs/west_random_power_mean.pdf}
%     \caption{ Power (random ITE) }  
% \end{subfigure}
% \begin{subfigure}[t]{0.24\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figs/west_fixed_disc_mean.pdf}
%     \caption{ Discovery (fixed ITE) } 
% \end{subfigure}
% \begin{subfigure}[t]{0.24\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figs/west_random_disc_mean.pdf}
%     \caption{ Discovery (random ITE) }  
% \end{subfigure}
% \caption{Power and discovery for fixed ITE (a-b) and random ITE (c-d)  with PAC-type procedure.}\label{fig:simu_ss_west_power}
% \end{figure}

% The demonstrated patterns are similar 
% to those in Section~\ref{subsubsec:simu_sens_mgn}. 
% Increased effect size 
% and more severe confounding lead to more discoveries. 
% However, confounding makes it harder to 
% identify positive ITEs at the correct robustness level. 
% Also, in general the PAC procedure has lower power than the 
% marginally valid procedure, since we pursue an intuitively 
% more difficult guarantee of high-probability error control. 

